Rank-Aware Speculative Sampling for Diffusion Draft Trees

Speculative sampling accelerates diffusion generation by verifying inexpensive draft states in parallel while preserving the target law. Recent tree-based methods allocate the parallel compute budget more effectively than single-chain drafts, as demonstrated by Diffusion Greedy Rejection Sampling (D-GRS). D-GRS generates $K$ conditionally independent candidates per node, and sequentially tests them in their generation order. Yet the sampled candidates admit an informative ranking without additional target-model evaluations. To exploit this, we introduce Rank-Aware Speculative Sampling (RASS), a verification rule for speculative draft trees based on rank-aware list coupling. RASS orders draft candidates along the proposal-target mean displacement and samples a rank with weights optimized to minimize total variation between the selected-proposal and target laws. Finally, the selected candidate is maximally coupled with the target, with residual correction ensuring exact sampling for any choice of rank weights. We evaluate RASS on a Gaussian-mixture target, unconditional pixel-space generation on FFHQ, conditional generation on CIFAR-10, and latent diffusion with Stable Diffusion 3.5 using COCO2014 prompts. Measured by the ratio of standard to speculative sampling's target-model evaluation counts, RASS improves on D-GRS across the evaluated settings, with gains reaching approximately 20% on CIFAR-10 at matched compute budgets.

==> figures/analysis/data/rank-simplex-plot.tex <==
% K = 3 rank-simplex figure. Load rank-simplex-preamble.tex first.
% CSV paths are relative to the main manuscript .tex file. If the CSVs live
% elsewhere, define \RankSimplexDir (with a trailing slash) before inputting
% this file, e.g. \def\RankSimplexDir{figures/rank-simplex/}.
% All numbers come from ../rank_simplex.py; nothing is computed here.
\begingroup
\providecommand{\RankSimplexDir}{}
% The mesh is streamed from file per panel: \pgfplotstableread is quadratic.
\pgfplotstableread[col sep=comma]{\RankSimplexDir rank-simplex-points.csv}\RankSimplexPoints

\definecolor{rankSimplexBlue}{HTML}{1F77B4}
\definecolor{rankSimplexOrange}{HTML}{FF7F0E}
\definecolor{rankSimplexPurple}{HTML}{9467BD}
\pgfplotsset{
  rank simplex dgrs/.style={color=rankSimplexBlue,line width=0.9pt},
  rank simplex path/.style={color=rankSimplexOrange,line width=1.2pt,
    line cap=round,dash pattern=on 0pt off 2.2pt},
  rank simplex unif/.style={only marks,mark=*,mark size=2.3pt,
    mark options={fill=white,draw=black,line width=0.4pt}},
  rank simplex max/.style={only marks,mark=triangle*,mark size=2.8pt,
    mark options={fill=rankSimplexPurple,draw=black,line width=0.4pt}},
  rank simplex star/.style={only marks,mark=rank simplex star,mark size=4pt,
    mark options={fill=rankSimplexOrange,draw=black,line width=0.4pt}},
}
\tikzset{
  rank simplex value/.style={anchor=north,inner sep=0pt,font=\scriptsize},
  rank simplex vertex/.style={inner sep=1pt,font=\scriptsize},
}

% One panel; #1 is the 0-based row of rank-simplex-points.csv, which also
% selects the shading column c#1 and the file rank-simplex-dgrs-#1.csv.
\newcommand{\RankSimplexPanel}[1]{%
  \addplot[patch,shader=interp,forget plot]
    table[col sep=comma,x=x,y=y,point meta=\thisrow{c#1}]
      {\RankSimplexDir rank-simplex-mesh.csv};
  \addplot[rank simplex dgrs,unbounded coords=jump,forget plot]
    table[col sep=comma,x=x,y=y] {\RankSimplexDir rank-simplex-dgrs-#1.csv};
  \draw[black,line width=0.4pt,line join=round]
    (axis cs:0,0) -- (axis cs:1,0) -- (axis cs:0.5,0.866025) -- cycle;
  \addplot[rank simplex path,forget plot]
    table[col sep=comma,x=x,y=y] {\RankSimplexDir rank-simplex-path.csv};
  \addplot[rank simplex unif,forget plot] coordinates {(0.5,0.288675)};
  \addplot[rank simplex max,forget plot] coordinates {(0.5,0.866025)};
  % Nodes are drawn when the axis closes, so each panel keeps its own copies
  % of the values (\RankSimplex<column>#1) rather than reusing one macro.
  \foreach \col in {delta,star_x,star_y,lab_unif,lab_max,lab_dgrs,lab_rass}{%
    \pgfplotstablegetelem{#1}{\col}\of\RankSimplexPoints
    \global\expandafter\let\csname RankSimplex\col#1\endcsname\pgfplotsretval
  }%
  \addplot[rank simplex star,forget plot] coordinates
    {(\csname RankSimplexstar_x#1\endcsname,\csname RankSimplexstar_y#1\endcsname)};
  \node[anchor=south,font=\small] at (axis cs:0.5,0.91)
    {$\delta=\csname RankSimplexdelta#1\endcsname$};
  \node[rank simplex value] at (axis cs:0.5,-0.13) {%
    \begin{tabular}{@{}l@{\hspace{0.9em}}l@{}}
      $\omega_{\mathrm{unif}}$: \csname RankSimplexlab_unif#1\endcsname &
      $\omega_{\mathrm{max}}$: \csname RankSimplexlab_max#1\endcsname \\
      D-GRS: \csname RankSimplexlab_dgrs#1\endcsname &
      RASS: \csname RankSimplexlab_rass#1\endcsname
    \end{tabular}};
}

\begin{tikzpicture}
  \begin{groupplot}[
    group style={group size=4 by 1,horizontal sep=0.015\linewidth},
    % Equal aspect: height/width = 0.94/1.04, the y/x ranges.
    scale only axis,width=0.2\linewidth,height=0.1808\linewidth,
    xmin=-0.02,xmax=1.02,ymin=-0.04,ymax=0.9,
    hide axis,clip=false,
    % ColorBrewer Greys, as matplotlib's "Greys".
    colormap={rank simplex greys}{rgb255=(255,255,255) rgb255=(240,240,240)
      rgb255=(217,217,217) rgb255=(189,189,189) rgb255=(150,150,150)
      rgb255=(115,115,115) rgb255=(82,82,82) rgb255=(37,37,37)
      rgb255=(0,0,0)},
    point meta min=0.5,point meta max=1,
  ]
    \nextgroupplot[
      legend to name=rankSimplexLegend,
      legend columns=5,
      legend style={draw=none,font=\scriptsize,cells={anchor=west},
        /tikz/every even column/.append style={column sep=0.9em}}
    ]
    \RankSimplexPanel{0}
    \node[rank simplex vertex,anchor=north] at (axis cs:0,-0.01) {$r=1$};
    \node[rank simplex vertex,anchor=north] at (axis cs:1,-0.01) {$r=2$};
    \node[rank simplex vertex,anchor=west] at (axis cs:0.55,0.866) {$r=3$};
    \addlegendimage{rank simplex unif}
    \addlegendentry{$\omega_{\mathrm{unif}}$ (RMC)}
    \addlegendimage{rank simplex max}
    \addlegendentry{$\omega_{\mathrm{max}}$}
    \addlegendimage{rank simplex star}
    \addlegendentry{RASS $\omega^\star$}
    \addlegendimage{rank simplex dgrs}
    \addlegendentry{D-GRS acceptance}
    \addlegendimage{rank simplex path}
    \addlegendentry{$\omega^\star(\delta)$ path}

    \nextgroupplot
    \RankSimplexPanel{1}

    \nextgroupplot
    \RankSimplexPanel{2}

    \nextgroupplot[
      colorbar,
      colorbar style={
        % Undo the panel settings the colour bar inherits.
        hide axis=false,xmin=0,xmax=1,clip=true,ytick pos=right,
        width=0.012\linewidth,
        xshift=0.005\linewidth,
        tick align=outside,
        major tick length=2pt,
        ytick={0.5,0.75,1},
        yticklabel style={font=\scriptsize,
          /pgf/number format/fixed,
          /pgf/number format/precision=2,
          /pgf/number format/fixed zerofill},
        ylabel={$\alpha_3(\delta;\omega)\,/\,\alpha^{\mathrm{up}}_3(\delta)$},
        ylabel style={font=\scriptsize},
      }
    ]
    \RankSimplexPanel{3}
  \end{groupplot}
  \node[anchor=north,inner sep=0pt] at ([xshift=0.0075\linewidth,yshift=-2.4em]group c2r1.south east)
    {\pgfplotslegendfromname{rankSimplexLegend}};
\end{tikzpicture}
\endgroup


==> figures/pixel-space/pixel-space-style.tex <==
% Local plot definitions; loaded inside the figure.
\pgfplotsset{compat=1.18}

\definecolor{pixelDGRS}{HTML}{1F77B4}
\definecolor{pixelRASS}{HTML}{FF7F0E}
\definecolor{pixelRMC}{HTML}{2CA02C}

% Discard other configurations while connecting the retained coordinates.
\pgfplotsset{
  pixel keep/.style 2 args={
    x filter/.append code={
      \getthisrow{#1}\pixelActual%
      \edef\pixelWanted{#2}%
      \ifx\pixelActual\pixelWanted\else
        \def\pgfmathresult{nan}%
      \fi
    }
  }
}

% Arguments: dataset, epsilon, saved method name, color.
\newcommand{\PixelCurve}[4]{%
  \addplot[draw=none,forget plot,name path=pixelLower,
    pixel keep={dataset}{#1},pixel keep={eps}{#2},pixel keep={rule}{#3}]
    table[x=B,y=ci_low] {\PixelData};
  \addplot[draw=none,forget plot,name path=pixelUpper,
    pixel keep={dataset}{#1},pixel keep={eps}{#2},pixel keep={rule}{#3}]
    table[x=B,y=ci_high] {\PixelData};
  \addplot[draw=none,fill=#4,fill opacity=0.16,forget plot]
    fill between[of=pixelLower and pixelUpper];
  \addplot[color=#4,thick,mark=*,mark size=1.4pt,forget plot,
    pixel keep={dataset}{#1},pixel keep={eps}{#2},pixel keep={rule}{#3}]
    table[x=B,y=speedup_mean] {\PixelData};
}

\newcommand{\PixelPanel}[2]{%
  \PixelCurve{#1}{#2}{d-grs}{pixelDGRS}%
  \PixelCurve{#1}{#2}{paws}{pixelRASS}%
  \PixelCurve{#1}{#2}{rmc}{pixelRMC}%
}

